A Principle for Global Optimization with Gradients

This work demonstrates the utility of gradients for the global optimization of certain differentiable functions with many suboptimal local minima. To this end, a principle for generating search directions from non-local quadratic approximants based on gradients of the objective function is analyzed. Experiments measure the quality of non-local search directions as well as the performance of a proposed simplistic algorithm, of the covariance matrix adaptation evolution strategy (CMA-ES), and of a randomly reinitialized Broyden-Fletcher-Goldfarb-Shanno (BFGS) method.

==> files-exp3/levy-vis.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
width=\linewidth,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x_1\)},
xmin=-0.5, xmax=999.5,
xtick style={color=black},
xtick={0,500,999},
xticklabels={-10,0,10},
y dir=reverse,
y grid style={darkgray176},
ylabel={\(\displaystyle x_2\)},
ymin=-0.5, ymax=999.5,
ytick style={color=black},
ytick={0,500,999},
yticklabels={10,0,-10}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=999.5, ymin=999.5, ymax=-0.5] {files-exp3/levy-vis-000.png};
\end{axis}

\end{tikzpicture}


==> files-exp3/rcigar-vis.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
width=\linewidth,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x_1\)},
xmin=-0.5, xmax=999.5,
xtick style={color=black},
xtick={0,500,999},
xticklabels={-10,0,10},
y dir=reverse,
y grid style={darkgray176},
%ylabel={\(\displaystyle x_2\)},
ymin=-0.5, ymax=999.5,
ytick style={color=black},
ytick={0,500,999},
%yticklabels={10,0,-10}
yticklabels={,,}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=999.5, ymin=999.5, ymax=-0.5] {files-exp3/rcigar-vis-000.png};
\end{axis}

\end{tikzpicture}


==> files-exp3/salomon-vis.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
width=\linewidth,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x_1\)},
xmin=-0.5, xmax=999.5,
xtick style={color=black},
xtick={0,500,999},
xticklabels={-10,0,10},
y dir=reverse,
y grid style={darkgray176},
%ylabel={\(\displaystyle x_2\)},
ymin=-0.5, ymax=999.5,
ytick style={color=black},
ytick={0,500,999},
%yticklabels={10,0,-10}
yticklabels={,,}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=999.5, ymin=999.5, ymax=-0.5] {files-exp3/salomon-vis-000.png};
\end{axis}

\end{tikzpicture}


==> files-exp3/siam-vis.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
width=\linewidth,
tick align=outside,
tick pos=left,
title={Visualization of \(\displaystyle f_{\mathrm{siam}}\)},
x grid style={darkgray176},
xlabel={\(\displaystyle x_1\)},
xmin=-0.5, xmax=999.5,
xtick style={color=black},
xtick={0,500,999},
xticklabels={-1,0,1},
y dir=reverse,
y grid style={darkgray176},
ylabel={\(\displaystyle x_2\)},
ymin=-0.5, ymax=999.5,
ytick style={color=black},
ytick={0,500,999},
yticklabels={1,0,-1}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=999.5, ymin=999.5, ymax=-0.5] {files-exp3/siam-vis-000.png};
\end{axis}

\end{tikzpicture}

